GNN4EEG: A Benchmark and Toolkit for Electroencephalography Classification with Graph Neural Network

Electroencephalography(EEG) classification is a crucial task in neuroscience, neural engineering, and several commercial applications. Traditional EEG classification models, however, have often overlooked or inadequately leveraged the brain's topological information. Recognizing this shortfall, there has been a burgeoning interest in recent years in harnessing the potential of Graph Neural Networks (GNN) to exploit the topological information by modeling features selected from each EEG channel in a graph structure. To further facilitate research in this direction, we introduce GNN4EEG, a versatile and user-friendly toolkit for GNN-based modeling of EEG signals. GNN4EEG comprises three components: (i)A large benchmark constructed with four EEG classification tasks based on EEG data collected from 123 participants. (ii)Easy-to-use implementations on various state-of-the-art GNN-based EEG classification models, e.g., DGCNN, RGNN, etc. (iii)Implementations of comprehensive experimental settings and evaluation protocols, e.g., data splitting protocols, and cross-validation protocols. GNN4EEG is publicly released at https://github.com/Miracle-2001/GNN4EEG.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       

==> algorithm.tex <==
\section{algorithm}

\begin{algorithm}
\caption{Real-time diversitify}
\label{alg:A}
\begin{algorithmic}
\STATE {\textbf{INPUT} 文档列表长度$k$, 查询$q$, 查询的subtopic集合$C(q)$，返回结果列表$R(q)$, 文档所属的subtopic集合$C(d)$, 查询在不同subtopic下的概率分布$P(c|q)$, 文档价值$V(d|q,c)$, 每次滑动的窗口大小$W_i$~($\sum_{1 \leq i \leq n(q)} W_i = k$), 用户满意度$Sat(d)$} 
\STATE {\textbf{set} $S = \emptyset, U(c|q,S)=P(c|q), i = 1$} 
\WHILE { $i<=n(q)$}
\FOR {$d \in R(q)$}
\STATE { $g(d|q,c,S) = \sum_{c \in C(d)} U(c|q,S)V(d|q,c)$}
\ENDFOR

\STATE {$ T^* = $ \textbf{argpartition}$(g(d | q, c, S) , W_i)$}
\STATE {$S= S\cup T^*, R(q) = R(q)\setminus T^*$}
\FOR {$d^* \in t^*$}
\STATE {$\forall c \in C(d^*), U(c|q,S) = (1-\frac{V(d^*|q, c)}{\sum_{c' \in C(d^*)}{V(d^*|q, c')}}*Sat(d^*))*U(c|q,S\setminus T^*)$ }
\ENDFOR
\ENDWHILE
\STATE {\textbf{return} $S$ }

\end{algorithmic}
\end{algorithm}


==> formula.tex <==

\section{formula}


$$
P_r(\theta_{k}^t=\theta|S_k^{t-1},F_k{t-1}
$$
$$
q_k^t(\theta_k^t)=\frac{Pr(R_k^t|\theta_k^t)Pr(\theta_k^t|S_k^{t-1}, F_k^{t-1})}{P_r(R_k^t|S_k^{t-1}, F_k^{t-1})}
$$
\begin{equation}
\begin{split}
	q_k^t(\theta_k^t)=q^0(\theta_k^t)[(1-\gamma)G^t(\theta_k^t)+...+(1-\gamma)^nG^{t-n+1}(\theta_k^t)]
\\ +\gamma^nG^t(\theta_k^t)...G^{t-n+1}(\theta_k^t)q_k^{t-n}(\theta_k^t)
\end{split}
\end{equation}




==> toolkit_old.tex <==
\section{toolkit}
Though with outstanding performances, studies of EEG classification via GNN, however, use their own evaluation settings based on customized sets of downstream tasks where the detailed process of adapting the models to these tasks is typically not accessible to the public. Moreover, source codes of these GNN models are either not accessible or difficult to reuse. Aiming to provide a flexible and easy-to-use framework for researchers and future studies, we build an integrated toolkit covering 3 validation protocols, 2 data splitting protocols and 4 GNN models interfaces. 

\subsection{Data Splitting Protocols}
Whether the subjects appearing in test set also appear in train set yields two different data splitting methods, i.e. intra-subject and cross-subject.

In intra-subject task, each subject's EEG signals appear both in train set and test set. On the contrary, in cross-subject task, train set 
 contains EEG signals from only part of subjects while other subjects' EEG signals are divided into test set.

\subsection{Validation Protocols}
Given different evaluation requirements, our toolkit provide 3 validation protocols, i.e. cross validation, nested cross validation and fixed epoch cross validation. Essentially, the difference among these 3 protocols lies in the selecting method of training epoch. 

\textbf{Cross Validation (CV).} Cross validation is a typical resampling method that uses different portions of the data to train and validate the model on different iterations. Conventionally, the data is divided into $K$ equal parts and the model is evaluated in $K$ training and validating iterations. On the $i$th iteration, the $i$th part of the data is chosen as validation set and others as train set. The maximum validation accuracy among all epochs is regarded as the evaluation result of the $i$th iteration and the average result among all iterations is reported. The algorithm of CV is presented in Algorithm.\ref{"alg.CV"}


% \begin{algorithm}
%   \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%   \Input{Dataset $\mathcal{D}$, GNN model $\mathcal{M}$, number of equal parts $K$, number of epochs $T$, other hyper-parameters $P$}
%   \Output{The averaged best validation accuracy among all $K$ iterations.}
%   \BlankLine
%   \For{$i=1$ to $K$}{
%     Split $\mathcal{D}$ into 
%     $\mathcal{D}^{train}_i$, $\mathcal{D}^{validation}_i$ 
    
%     Initialize $\mathcal{M}$ via hyper-parameters $P$
    
%     \For{$j=1$ to $T$}{
%         Train $\mathcal{M}$ on $\mathcal{D}^train_i$ for an epoch
        
%         Compute the accuracy $Acc_j$ for $\mathcal{M}$ on  $\mathcal{D}^{validation}_i$ 
%     }
%     Compute $Result_i=max\{{Acc_1,Acc_2,...,Acc_T}\}$    
%     % Select the best accuracy among all $Accuracy_j$ where $j=1,2,...,T$ as 
%   }
%   Compute $Avg=\frac{1}{K}\sum_{i=1}^{K}Result_i$
  
%   \textbf{Return} $Avg$
%   \caption{The procedure of CV}
%   \label{"alg.1"}

% \end{algorithm}

\begin{algorithm}
	%\textsl{}\setstretch{1.8}
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\caption{The procedure of CV}
        \label{"alg.CV"}
	\begin{algorithmic}[1]
            \REQUIRE{Dataset $\mathcal{D}$, GNN model $\mathcal{M}$, number of equal parts $K$, number of epochs $T$, other hyper-parameters $P$}
            \ENSURE{The averaged best validation accuracy among all $K$ iterations.}
            % \BlankLine
            \FOR{$i=1$:$K$}
            \STATE Initialize $\mathcal{M}$ via hyper-parameters $P$
            \STATE Split $\mathcal{D}$ into 
            $\mathcal{D}^{train}_i$, $\mathcal{D}^{validation}_i$ 
            \FOR{$j=1$:$T$}
             \STATE Train $\mathcal{M}$ on $\mathcal{D}^{train}_i$ for an epoch
             \STATE Compute the validation accuracy $Acc_{i,j}$ for $\mathcal{M}$ on  $\mathcal{D}^{validation}_i$ 
            \ENDFOR
            \ENDFOR
            \FOR{$i=1$:$K$}
             \STATE Compute $MAX_i=max\{{Acc_1,Acc_2,...,Acc_T}\}$
            \ENDFOR
		\STATE Compute $AVG=\frac{1}{K}\sum_{i=1}^{K}MAX_i$
		\RETURN  $AVG$
	\end{algorithmic}  
\end{algorithm}

Note that in cross validation method, the training epoch selected according to the best validation accuracy can vary in different iterations. However, considering the curve with intensive fluctuation during each training progress showed in Fig.\ref{acc_and_loss}, the accuracy acquired by simply choosing the best epoch may introduce unpredictable random factor, decreasing the confidence level of the result.
% In other words, the best validation accuracy on an intensive fluctuation curve can not properly represent the generalization ability.

\textbf{Fixed Epoch Cross Validation (FCV).} To address the above issue, a fixed epoch cross validation is proposed, in which the number of epoch among all iterations is fixed and selected according to the best cross validation accuracy averaged over $K$ folds. Algorithm.\ref{"alg.FCV"} summarizes the procedure of FCV.

\begin{algorithm}
	%\textsl{}\setstretch{1.8}
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\caption{The procedure of FCV}
        \label{"alg.FCV"}
	\begin{algorithmic}[1]
            \REQUIRE{Same as Algorithm.\ref{"alg.CV"}}
            \ENSURE{The best averaged validation accuracy among all $T$ epochs and the corresponding fixed epoch number.}
            \STATE Compute $Acc_{i,j}$ like Algorithm.\ref{"alg.CV"}
            \FOR{$j=1$:$T$}
            \STATE Compute $AVG_j=\frac{1}{K}\sum_{i=1}^{K}Acc_{i,j}$
            \ENDFOR
		\STATE Compute $MAX=max\{{AVG_1,AVG_2,...,AVG_T}\}$
            \STATE Compute $FixedEpoch=argmax\{{AVG_1,AVG_2,...,AVG_T}\}$
		\RETURN  $MAX,FixedEpoch$
	\end{algorithmic}  
\end{algorithm}

\textbf{Nested Cross Validation (NCV).} Evaluation methods above choose the hyper-parameters (epoch number) according to the performance on validation set, but still report the accuracy on the same data set, thus leading to data leakage. So in order to evaluate the generalization ability in a more appropriate manner, the nested cross validation is applied.

Based on CV,  NCV further divides the train set of each iteration into another $K'$ equal parts, introducing an "inner" and "outer" cross validation manner. The "inner" is responsible for selecting the best epoch number and the "outer" averages the accuracy over $K$ folds. Namely, NCV introduces not only train set and validation set, but also test set, thus providing a more reliable estimate of the generalization ability. The pseudo-code is shown in Algorithm .\ref{"alg.NCV"}

\begin{algorithm}
	%\textsl{}\setstretch{1.8}
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\caption{The procedure of NCV}
        \label{"alg.NCV"}
	\begin{algorithmic}[1]
            \REQUIRE{Number of inner partition $K'$, others same as Algorithm.\ref{"alg.CV"}}
            \ENSURE{The averaged test accuracy among all $K$ iterations.}
            \FOR{$i=1$:$K$}
            \STATE Split $\mathcal{D}$ into 
            $\mathcal{D}^{test}_i$, $\mathcal{D}^{train}_i$ 
            \STATE Call the FCV algorithm (i.e. Algorithm.\ref{"alg.FCV"}) where $\mathcal{D}$ is set as $\mathcal{D}^{train}_i$ and $K$ is set as $K'$ (other inputs are the same as NCV)
            \STATE Receive $FixedEpoch$ from the FCV algorithm 
            \STATE Initialize $\mathcal{M}$ via hyper-parameters $P$
             \FOR{$j=1$:$FixedEpoch$}
             \STATE Train $\mathcal{M}$ on $\mathcal{D}^{train}_i$ for an epoch
            \ENDFOR
            \STATE Compute the test accuracy $Acc_i$ for $\mathcal{M}$ on  $\mathcal{D}^{test}_i$ 
            \ENDFOR
		\STATE Compute $AVG=\frac{1}{K}\sum_{i=1}^{K}Acc_{i}$
		\RETURN  $AVG$
	\end{algorithmic}  
\end{algorithm}

\subsection{GNN for EEG Classification}
In this section, we give a brief introduction about graph convolution network(GCN) as well as the four GNN model provided in our toolkit, i.e. DGCNN, RGNN, SparseDGCNN and HetEmotionNet.

Formally, a graph can be defined as $G=(V,E)$, where $V$ denotes the node set and $E$ denotes the edge set. The input feature on $V$ can be represented as a matrix $X\in \mathbb{R}^{n*d}$ , where $n=|V|$ and $d$ denotes the input feature dimension. The edge weight of $E$ can be represented by a weighted adjacency matrix $A\in \mathbb{R}^{n*n}$ with self-loops. Furthermore, we can calculate the diagonal  degree matrix $D$ of $A$ via $D_{ii}=\sum_j A_{ij}$. 
\subsubsection{GCN}
GCN, a kind of GNN, is useful when aggregating and combining features extracted from EEG signals in an end-to-end fashion. In general, the forward propagation of one GCN layer can be written as follows.
\begin{equation}
\label{GCN_forward}
H^{l+1}=\sigma(D^{-\frac{1}{2}}AD^{-\frac{1}{2}}H^lW^l) 
\end{equation}
where l=0,1,...,L-1,L denotes the number of layers, with $H^0=X$. For each layer $l$, $\sigma$ represents a non-linear function and $W^l$ represents a weight matrix.

\subsubsection{DGCNN}
DGCNN model consists of a graph filtering layer (can be approximated as Eq.\ref{GCN_forward}), a convolution layer, an activation layer and a fully connected layer. Note that the adjacency matrix $A$ in DGCNN is optimized during training and $A_{ii}\ge 0$ is always held. Though DGCNN is simple enough, it still outperforms other models like SVM and GSCCA on certain databases.

\subsubsection{RGNN}
Focusing on the poor performance while applying GCN models on cross-subject tasks and noisy labels conditions in EEG emotion recognition, RGNN proposes two regularizers named NodeDAT and EmotionDL. In contrary of DGCNN, RGNN introduced negative number to represent global connection. 

\subsubsection{SparseDGCNN}
Different from RGNN, SparseDGCNN model aims to improve the sparseness of the adjacency matrix during training by imposing a sparseness constraint. Moreover, this model also applies a forward-backward splitting met,hod to ensure the training process converges. 

\subsubsection{HetEmotionNet}
HetEmotionNet use a novel two-stream heterogeneous graph recurrent neural network to capture both spatial-spectral and spatial-temporal features in multi-modal physiological signals. Graph Transformer Network(GTN) and Gated Recurrent Unit(GRU) are components responsible for heterogeneity graph aggregation and recurrent features extraction, respectively.

\subsection{Examples and Uses}

Note that data preprocessing (e.g. frequency feature extraction, data smooth, etc.) methods are not provided, so users should apply these methods on their own if necessary. 

\subsubsection{Evaluation Protocol Selection}
inter/intra
cv,fcv,ncv
lr,l1reg,l2reg
device
\subsubsection{GNN Model Usage}
build model:
n-class,n-nodes,n-features,n-hiddens,n-layers
dropout

train:

predict:

